Multigrid reduction preconditioning framework for coupled processes in porous and fractured media

Many subsurface engineering applications involve tight-coupling between fluid flow, solid deformation, fracturing, and similar processes. To better understand the complex interplay of different governing equations, and therefore design efficient and safe operations, numerical simulations are widely used. Given the relatively long time-scales of interest, fully-implicit time-stepping schemes are often necessary to avoid time-step stability restrictions. A major computational bottleneck for these methods, however, is the linear solver. These systems are extremely large and ill-conditioned. Because of the wide range of processes and couplings that may be involved--e.g. formation and propagation of fractures, deformation of the solid porous medium, viscous flow of one or more fluids in the pores and fractures, complicated well sources and sinks, etc.--it is difficult to develop general-purpose but scalable linear solver frameworks. This challenge is further aggravated by the range of different discretization schemes that may be adopted, which have a direct impact on the linear system structure. To address this obstacle, we describe a flexible framework based on multigrid reduction that can produce purely algebraic preconditioners for a wide spectrum of relevant physics and discretizations. We demonstrate its broad applicability by constructing scalable preconditioners for several problems, notably: a hybrid discretization of single-phase flow, compositional multiphase flow with complex wells, and hydraulic fracturing simulations. Extension to other systems can be handled quite naturally. We demonstrate the efficiency and scalability of the resulting solvers through numerical examples of difficult, field-scale problems.

==> Section2_Formulation.tex <==
\section{Linear Solver Overview\todo{NC:do we need the two subsections?}} \label{sec:formulation}
%\subsection{Block Linear Systems}
%These problems are modeled by a set of tightly coupled PDEs. For example, in compositional multiphase flow, each component is modeled with a mass conservation equation and the coupling between the components are modeled by the mass exchange terms between them. In the case of hydraulic fracturing, the equation for mass conservation of the fluid inside the fracture is coupled with the elasticity equation governing the deformation of the porous medium. In general, we seek solutions to the following problem
%\begin{align}
%    \mathcal{F}_i(\mathbf{u}) = 0, \hspace{5mm} i = 1, 2, \dots, M \label{eq:pde_system}
%\end{align}
%in which $\mathcal{F}_i$ is a PDE, $\mathbf{u}$ is vector of variables representing the physical quantities of interest, and $M$ is the number of PDEs in the system. For example, for immiscible two-phase flow and black oil models, we have $M = 2$ and $M = 3$, respectively. The particular form of \cref{eq:pde_system} for our applications are discussed in \cref{sec:hydraulic_fracturing,sec:compositional_models}.

%Due to the tightly coupled nature of the system, fully-implicit approaches are the methods of choice. In particular, the backward Euler method is popular scheme for subsurface applications. For spatial discretizations,  finite element and finite volume methods can be employed as appropriate. For example, in our applications, the momentum balance equation for elasticity is discretized with a finite element scheme, while the equations for fluid flow are typically discretized using a finite volume method. After discretizations, collecting all the degrees of freedom associated with a field into an algebraic vector $\mathbf{u}=(u_1, u_2, \dots, u_M)^T$ leads to a set of coupled residual equations
%\begin{equation}
%r(\mathbf{u}^k,\mathbf{u}^{k-1}) = 
%\begin{pmatrix}
%r_\text{PDEs}\\
%r_\text{constraints}
%\end{pmatrix} = 0 \,,
%\end{equation}
%where $\mathbf{u}^k, \mathbf{u}^{k-1}$ are the solution vectors at the current and previous timesteps, respectively. At a given timestep, these equations are solved using Newton's method, with a backtracking algorithm to improve convergence robustness.  Ignoring the superscript for the time step, given a previous estimate of the solution $\mathbf{u}^{i-1}$, a Newton iteration provides an improved estimate $\mathbf{u}^{i}$ as follows.
%\begin{align}
%\text{solving} \quad & A^{i-1} \Delta {\mathbf{u}} = - {r}^{i-1} \,, \\
%\text{updating} \quad & \mathbf{u}^i = \mathbf{u}^{i-1} + \gamma \Delta %\mathbf{u} \,.
%\end{align}
%Here, $A = \partial {r} / \partial {x}$ is the Jacobian of the nonlinear system, and $\gamma \in (0,1]$ is a backtracking parameter that limits the step length in direction $\Delta {\mathbf{u}}$ to ensure a residual reduction.  The iterations are terminated when the residual norm drops below a desired nonlinear convergence tolerance, $\|  r  \| < \epsilon$.  In general, the matrix $A$ has the following block structure
In this work, we focus on solving $\mathcal{B}\times \mathcal{B}$\todo{NC: $M$ is extensively used for preconditioners in this paper. We should use another letter, maybe $B$ for block.} block linear systems of the form
\begin{linenomath}
\begin{align}
A x &= b,
&
A &=
\begin{pmatrix}
  A_{11} & A_{12} & \cdots & A_{1M} \\
  A_{21} & A_{22} & \cdots & A_{2M} \\
  \vdots & \vdots & \ddots & \vdots \\
  A_{M1} & A_{M2} & \cdots & A_{MM}
\end{pmatrix},
&
x &=
\begin{pmatrix}
  x_1 \\
  x_2 \\
  \vdots \\
  x_M
\end{pmatrix},
&
b &= 
\begin{pmatrix}
  b_1 \\
  b_2 \\
  \vdots \\
  b_M
\end{pmatrix}, \label{eq:linear_system}
\end{align}
\end{linenomath}
arising from fully implicit simulation of dynamic subsurface processes in porous and fracture media, e.g. single-physics problems in mixed form or tightly-coupled multiphysics problems.
%
Here, $A_{ij}$ with $i, j = 1, 2, \dots, \mathcal{B}$ are block matrices of size $N_i \times N_j$ induced by a physics-based partitioning of the the unknowns collected in $x$ by field type, with $N_i$ (respectively $N_j$) the numbers of degrees of freedom associated with the physical quantities $x_i$ (respectively $x_j$).
%
%Such linear systems appear frequently in numerical simulations of flow in porous and fractured media.



%\textcolor{red}{
%\todo{NC:I would drop the rest of this subsection} To give an example, in the case of scalar PDEs such as incompressible single-phase flow, a mixed finite-element discretization results in a $2\times 2$ block matrix representing a saddle-point problem of face-based Darcy's fluxes and cell-based pressures; in a mixed-hybrid finite-element method, the introduction of a Lagrange multiplier for face-based pressure produces a symmetric indefinite $3\times 3$ block matrix that can be solved using a Schur-complement approach \cite{Lie19}.
%
%In this work, we solve a linear system coming from a hybrid MFD method applied to a compressible single-phase flow, whose block structure is described in \cref{subsec:hybrid_mfvm}.
%}

%\textcolor{red}{
%Mixed and hybrid discretization methods for scalar PDEs only represent a small area that solution of block systems in \cref{eq:linear_system} is needed.
%
%The most common case is, however, modeling multiphysics problems that are governed by a set of tightly coupled PDEs.
%
%In this case, the number of blocks in $A$ usually depends on the number of PDEs in the system and the number of physical regions that have different geometric representations.
%
%For instance, in hydraulic fracturing with single-phase flow, $A$ is a $2\times 2$ block system corresponding to the reservoir and the fracture regions, which are represented by a three-dimensional volume mesh and a two-dimensional planar mesh, respectively.
%
%For compositional flow, the number of blocks is determined by the number of mass conservation and control equations for the components of the flow in the reservoir and wells.
%
%Detailed description of the block systems for these two applications are presented in %\cref{subsec:hydraulic_fracturing,subsec:compositional_flow}.
%}

%\subsection{Solution Method}
For large dimensional linear systems global iterative solution strategies
are the method of choice, typically Krylov subspace methods \cite{Saa03}.
%
Preconditioning is the key for enabling efficient solution by such methods \cite{Ben02,Wat15}.
%
The idea of preconditioning is to transform the original system of equations, through a preconditioner, into an equivalent system that has a lower condition number.
%
We solve the block system in \cref{eq:linear_system} using a preconditioned Krylov solver, e.g. the generalized minimal residual method (GMRES) \cite{Saad86}.
%
%
For example, using right preconditioning,
%instead of solving the linear system
%\begin{linenomath}
%\begin{align}
%A x = b,
%\end{align}
%\end{linenomath}
%we solve 
the original system \cref{eq:linear_system} is replaced by 
\begin{linenomath}
\begin{align}
AM^{-1} y = b,
\end{align}
\end{linenomath}
where $Mx = y$. The key idea is to find a matrix $M$ that can approximate $A$ well, while at the same time the action of $M^{-1}$ is cheap to compute.

\par Here, to construct the matrix $M$, we focus on multilevel methods, which can be algorithmically and computationally optimal.
%
That is, they require $\mathcal{O}(N)$ complexity where $N$ is the number of degrees of freedom, and exhibit good parallel scaling on large parallel architectures. 
%
%Multigrid is one such algorithm and is among the most efficient and scalable methods for solving large sparse linear systems. There are two main variants of multigrid: \textit{geometric multigrid} (GMG) and \textit{algebraic multigrid} (AMG). State-of-the-art GMG solvers include implementations in the UG package \cite{Reiter13}, \textit{hypre} \cite{Falgout02}, and an agglomeration-based variant in PETSc \cite{Baley12}. For GMG methods, one needs to explicitly construct a hierarchy of grids. This process is very challenging for problems with complex geometry that rely on unstructured grids. The Hierarchical Hybrid Grids (HHG) method \cite{Gmeiner15} mitigates some of these challenges. In contrast, AMG methods construct the computational grids from the input matrix, eliminating the need for explicit construction of grid hierarchy. High performing AMG packages include BoomerAMG \cite{Henson00} in the \textit{hypre} \cite{Falgout02} library, ML \cite{Gee06} in Trilinos \cite{Heroux05}, and an AMG solver for heterogeneous coefficients from the DUNE project \cite{Blatt11}. 

%Even though these solvers are extremely efficient, capable of scaling to hundreds of thousands of cores, their applicability is limited to scalar problems, i.e. single-block linear systems. For tightly coupled problems that require solution of multiple-block linear systems, off-the-shelf applications of these methods usually result in non-convergent or non-optimal results. Thus, much of the work in developing solver strategies for coupled problems has focused on block preconditioners with approximate Schur complement, also called physics-based strategies. This approach utilizes knowledge of the specific physical processes involved to break the tightly coupled systems into smaller sub-problems whose properties are well-studied. Specifically, these sub-problems could take the form of an elliptic, hyperbolic, or parabolic PDE, to which appropriate solver techniques can be applied. As such, block preconditioners are highly specialized and domain-specific, making them unsuitable as a general solver. 

There have been efforts to facilitate development of block preconditioners by combining existing single-physics solvers. For example, PETSc's `PCfieldsplit' functionality allows one to compose sophisticated block preconditioners by splitting the solution vector into physical fields. However, for systems with a large number of blocks such as compositional flow, this task still requires a significant effort, since all of the components of such preconditioners, i.e. the factorization of the global block system, approximations of the Schur complements, solver choices for each block, etc., needs to be defined by the user. The Teko package in the Trilinos project provides a tool for automated construction of block preconditioners that are more tailored to the Navier-Stokes equation. In this work, we present a framework that balances the flexibility of PETSc’s `PCFieldSplit' and black-box usage of Teko to specifically target problems in porous and fractured media using \textit{multigrid reduction} (MGR). MGR has been proposed as a scalable strategy for preconditioning multiphysics problems and it has been successfully applied to multiphase flow in porous media \cite{Wang17}, with phase transitions \cite{Bui18}, and multiphase flow coupled with poromechanics \cite{Bui20}.


%In this work, we adopt the MGR framework to develop reduction-based strategies that are efficient and scalable for a hybrid MFD discretization of single-phase flow, compositional flow with wells, and hydraulic fracturing. 
In this work, we demonstrate flexibility, robustness and scalability of the MGR framework focusing on three relevant models extensively used in computational geosciences: 
%
(i) compressible single-phase flow discretized by a hybrid mimetic finite difference method (\cref{subsec:hybrid_mfvm});
%
(ii) two-phase, two-component compositional flow with wells discretized by a classical two-point flux approximation (TPFA) finite volume method (\cref{subsec:compositional_flow}); and 
%
(iii) field-scale hydraulic fracturing using a fully coupled mixed finite element/finite volume approach (\cref{subsec:hydraulic_fracturing}).
%
In the next section, we briefly review the main ideas of MGR and describe how it is generalized to solve the system specified in \cref{eq:linear_system}.

